Real-time jam-session support system

We propose a method for the problem of real time chord accompaniment of improvised music. Our implementation can learn an underlying structure of the musical performance and predict next chord. The system uses Hidden Markov Model to find the most probable chord sequence for the played melody and then a Variable Order Markov Model is used to a) learn the structure (if any) and b) predict next chord. We implemented our system in Java and MAX/Msp and compared and evaluated using objective (prediction accuracy) and subjective (questionnaire) evaluation methods.

==> Makefile <==
all:
	xelatex -shell-escape dissertation.tex

bib:
	xelatex -shell-escape dissertation.tex
	bibtex dissertation
	xelatex -shell-escape dissertation.tex
	xelatex -shell-escape dissertation.tex

wordcount:
	pdftotext dissertation.pdf - | egrep -E '\w\w\w+' | wc -w


==> tmp.tex <==
\section{Chords}

Lets recall what a chord is. Chord is a group of 3 or more notes that are played simultaneously. The name of the chord reveals
it's structure and it's mainly named after the type of the intervals of it's components.  For example a chord with a 3rd interval of 3 semitones
is named minor whereas a 3rd of 4 semitones major. 

[image illustrating chord intervals and construction]

The most basic type of chord is a triad, which is a chord which consist of 3 notes. The root note, the 3rd and the 5th. 
The main triad qualities are the following :
major
minor
augmented
minished
[table with chords]

% http://en.wikipedia.org/wiki/Chord_(music)#Chord_characteristics

==> tmps/Bayesian_network.tex <==

\begin{figure}[!h]
\centering
\includegraphics{../figures/bayesian_net.pdf}
\caption{Bayesian network used for melody prediction and chord infernce}
\label{factor_graph}
\end{figure}

Given that $c_{t} = C_{t}, c_{t-1}=C_{t-1},n_{t} = N_{t}$ and $n_{t-1}=N_{t-1}$ we want to find
\begin{eqnarray*}
Pr(c_{t+1}|c_{t}, c_{t-1},n_{t},n_{t-1}) &=& \sum_{n_{t+1}}{  Pr(c_{t+1},n_{t+1}|c_{t}, c_{t-1}, n_{t},n_{t-1}) } \\
&=& \sum_{n_{t+1}}{ \frac{Pr(c_{t+1},c_{t}, c_{t-1},n_{t+1}, n_{t},n_{t-1})}{Pr(c_{t}, c_{t-1},n_{t},n_{t-1} )} } \\
&=& \sum_{n_{t+1}}{ \frac{
	Pr(c_{t+1}|c_{t},c_{t-1},n_{t+1})
	Pr(c_{t})
	Pr(c_{t-1})
	Pr(n_{t+1}|n_{t},n_{t-1} ) 
	Pr(n_{t})
	Pr(n_{t-1})
	}
	{
	Pr(c_t)
	Pr(c_{t-1})
	Pr(n_{t})
	Pr(n_{t-1})
	} }\\
\end{eqnarray*}
However, $Pr(c_t) \neq 0, Pr(c_{t-1}) \neq 0, Pr(n_t) \neq 0,$ and $Pr(n_{t-1}) \neq 0$ since we used Laplace correction during the training. Thus
\begin{eqnarray*}
Pr(c_{t+1}|c_{t}, c_{t-1},n_{t},n_{t-1}) &=& \sum_{n_{t+1}}{
		Pr(c_{t+1}|c_t,c_{t-1},n_{t+1})
		Pr(n_{t+1}|n_t,n_{t-1})
	}
\end{eqnarray*}
To infer the next chord we have to find the argument that maximize this probability. 
\begin{eqnarray*}
c_{t+1}=\arg\max_{c_{t+1}}{ Pr(c_{t+1}|c_{t}, c_{t-1},n_{t},n_{t-1})} &=& \arg\max_{c_{t+1}}{\sum_{n_{t+1}}{
		Pr(c_{t+1}|c_t,c_{t-1},n_{t+1})
		Pr(n_{t+1}|n_t,n_{t-1})
	 } }
\end{eqnarray*}


==> tmps/factor_graph.tex <==

\begin{figure}[!h]
\centering
\includegraphics{../figures/fractor_graph.pdf}
\caption{factor graph of the Bayesian network}
\label{factor_graph}
\end{figure}

To compute $p(c_{t+1})$ we have to marginalize over $c_t, c_{t-1}, n_{t+1}, n_t, n_{t-1}$ thus :
\[
p(c_{t+1})=\sum_{c_t, c_{t-1}, n_{t+1}, n_t, n_{t-1} }{p(c_t)p(c_{t-1})p(n_t)p(n_{t-1})p(c_{t+1}|c_t,c_{t-1},n_{t+1})p(n_{t+1}|n_t,n_{t-1})}
\]
which has $O(C^2N^3)$ complexity. However, using a method based on factor graphs and message passing we can reduce the time complexity.

\textbf{Message Passing} \\
The equations derived from figure \ref{factor_graph} are the following:
\begin{eqnarray*}
\mu_{f_2 \rightarrow c_{t-1}}(c_{t-1}) &=& f_2(c_{t-1}) \\
\mu_{c_{t-1} \rightarrow f_5}(c_{t-1})&=&\mu_{f_2 \rightarrow c_{t-1}}(c_{t-1})=f_2(c_{t-1}) \\
\mu_{f_1 \rightarrow c_{t}}(c_{t})&=&f_1(c_{t}) \\
\mu_{c_{t} \rightarrow f_5}(c_{t})&=&\mu_{f_1 \rightarrow c_{t}}(c_{t})=f_1(c_{t}) \\
\mu_{f_5 \rightarrow c_{t+1}}(c_{t+1})&=&\sum_{c_{t}, c_{t-1}, n_{t+1}}{f_{5}(c_{t},c_{t-1}, n_{t+1}) \mu_{c_{t-1} \rightarrow f_5}(c_{t-1})} \mu_{c_{t} \rightarrow f_5}(c_{t}) \mu_{n_{t+1} \rightarrow f_5}(n_{t+1})\\
\mu_{f_3 \rightarrow n_t}(n_t)&=& f_3(n_t)\\
\mu_{n_t \rightarrow f_6}(n_t)&=&\mu_{f_3 \rightarrow n_t}(n_t)= f_3(n_t)\\
\mu_{f_4 \rightarrow n_{t-1}}(n_{t-1})&=&f_4(n_{t-1})\\
\mu_{n_{t-1} \rightarrow f_4}(n_{t-1})&=&\mu_{f_4 \rightarrow n_{t-1}}(n_{t-1})=f_4(n_{t-1})\\
\mu_{f_6 \rightarrow n_{t+1}}(n_{t+1})&=&\sum_{n_{t-1},n_t}{f_6(n_{t+1}, n_t, n_{t-1})} \mu_{n_t \rightarrow f_6}(n_t)\mu_{n_{t-1} \rightarrow f_6}(n_{t-1})\\
\mu_{n_{t+1} \rightarrow f_5}(n_{t+1})&=&\mu_{f_6 \rightarrow n_{t+1}}(n_{t+1})
\end{eqnarray*}
$f_i$ is simple look-up table.

The probability $p(c_{t+1})$ is computed by computing $\mu_{f_5 \rightarrow c_{t+1}}(c_{t+1})$. The complexity of belief propagation
is $O(N C^2+N^2)$, where $N=12$ and $C=60$.


==> yo.tex <==
\begin{minted}{python}
	import test
	
	def test(self):
		pass
\end{minted}
